Rethinking Graph Contrastive Learning through Relative Similarity Preservation

Graph contrastive learning (GCL) has achieved remarkable success by following the computer vision paradigm of preserving absolute similarity between augmented views. However, this approach faces fundamental challenges in graphs due to their discrete, non-Euclidean nature -- view generation often breaks semantic validity and similarity verification becomes unreliable. Through analyzing 11 real-world graphs, we discover a universal pattern transcending the homophily-heterophily dichotomy: label consistency systematically diminishes as structural distance increases, manifesting as smooth decay in homophily graphs and oscillatory decay in heterophily graphs. We establish theoretical guarantees for this pattern through random walk theory, proving label distribution convergence and characterizing the mechanisms behind different decay behaviors. This discovery reveals that graphs naturally encode relative similarity patterns, where structurally closer nodes exhibit collectively stronger semantic relationships. Leveraging this insight, we propose RELGCL, a novel GCL framework with complementary pairwise and listwise implementations that preserve these inherent patterns through collective similarity objectives. Extensive experiments demonstrate that our method consistently outperforms 20 existing approaches across both homophily and heterophily graphs, validating the effectiveness of leveraging natural relative similarity over artificial absolute similarity.

==> 2.5-theory.tex <==
\section{Theoretical Analysis}
\label{sec:theory}

Our empirical study in Section~\ref{sec:empirical} reveals two intriguing patterns in graph label similarity: a universal decay trend where label similarity decreases with distance, and distinct decay patterns between homophily and heterophily graphs. To provide theoretical understanding of these phenomena, we analyze label propagation through the lens of random walks on graphs~\cite{lovasz1993random}, a natural framework that captures how label information diffuses along network structure.
Consider a random walk starting from a node with label $i$ in a graph with $c$ distinct labels. While traditional random walks operate at the node level with transition probability $P_{uv} = A_{uv}/\text{deg}(u)$, we analyze the label transition dynamics by aggregating node-level transitions between different label classes. Let $p_k(j|i)$ denote the probability of reaching a node with label $j$ after $k$ steps, starting from any node with label $i$. We define the Label Consistency (LC) at step $k$ as $p_k(i|i)$, measuring the probability of returning to a node with the same label. The transition between labels is characterized by a label-level transition matrix $T$, where $T_{ij}$ represents the probability of transitioning from any node with label $i$ to any node with label $j$:

\begin{equation}
\label{eq:transition_prob}
T_{ij} = \frac{\sum_{u:l(u)=i}\sum_{v:l(v)=j}A_{uv}}{\sum_{u:l(u)=i}\text{deg}(u)}.
\end{equation}

We establish the following fundamental results about label distribution dynamics:

\begin{theorem}[Label Distribution Convergence]
\label{thm:convergence}
For a connected graph where each node has a self-loop, there exists a unique probability distribution $\pi$ (where $\pi_j = \frac{\sum_{u:l(u)=j}\text{deg}(u)}{\sum_v \text{deg}(v)}$) such that:
\begin{equation}
\lim_{k \to \infty} p_k(j|i) = \pi_j,
\end{equation}
moreover, the convergence is exponential:
\begin{equation}
|p_k(j|i) - \pi_j| \leq C\lambda^k,
\end{equation}
where $C > 0$ and $\lambda < 1$ are constants determined by the graph structure.
\end{theorem}

\begin{proof}[Proof Sketch]
The key is showing that $T$ satisfies essential Markov chain properties: row-stochasticity follows from normalization, graph connectivity ensures irreducibility, and self-loops guarantee aperiodicity. The Perron-Frobenius theorem~\cite{levin2017markov} then yields the unique stationary distribution $\pi$ and exponential convergence rate bound. Full proof in Appendix~\ref{appendix:theory:proof_convergence}.
\end{proof}

This stationary distribution $\pi$ has a clear physical interpretation: $\pi_j$ represents the proportion of edges connected to nodes with label $j$ in the graph, serving as the natural limit for label transition probabilities and characterizing the structural importance of different labels in terms of their connectivity patterns. Based on this convergence theorem, we derive:

\begin{corollary}[Label Consistency Decay]
\label{cor:lc_decay}
The Label Consistency $LC(k) = p_k(i|i)$ exhibits a decay pattern where:
\begin{equation}
\begin{aligned}
&LC(0) = 1, \\
&\lim_{k \to \infty} LC(k) = \pi_i < 1, \\
&|LC(k) - \pi_i| \leq C\lambda^k.
\end{aligned}
\end{equation}
\end{corollary}

\begin{proof}[Proof Sketch]
$LC(0)=1$ by definition as we start at a node with label $i$. As $k\to\infty$, Theorem~\ref{thm:convergence} gives the limit $\pi_i$. Graph connectivity ensures $\pi_i<1$ since some edges must connect to nodes with other labels, making $\sum_{u:l(u)=i}\text{deg}(u) < \sum_v \text{deg}(v)$. Exponential decay follows from spectral decomposition of $T^k$. Detailed proof in Appendix~\ref{appendix:theory:proof_decay}.
\end{proof}

While both homophilic and heterophilic graphs exhibit this universal LC decay as shown in Section~\ref{sec:empirical}, their decay patterns differ significantly---homophilic graphs (8 instances shown in Figure~\ref{fig:lc_decay}a) demonstrate smooth, near-monotonic decay, while heterophilic graphs (3 instances shown in Figure~\ref{fig:lc_decay}b) show oscillatory patterns. To provide theoretical insight into these distinct behaviors, we analyze a simplified two-label case:

\begin{proposition}[Decay Pattern Characterization]
\label{prop:decay_patterns}
In a two-label simplified model, homophilic graphs yield transition matrices of the form $T \approx \begin{bmatrix}p & 1-p \\ 1-p & p\end{bmatrix}$ with $p \gg 0.5$, leading to positive second eigenvalue; while heterophilic graphs yield $T \approx \begin{bmatrix}1-p & p \\ p & 1-p\end{bmatrix}$ with $p \gg 0.5$, resulting in negative second eigenvalue, explaining their smooth versus oscillatory decay patterns.
\end{proposition}

\begin{proof}[Proof Sketch]
For homophilic graphs, dominant diagonal entries $T_{ii}$ lead to positive $\lambda_2 = 2p-1$. For heterophilic graphs, dominant off-diagonal entries $T_{ij}$ ($i \neq j$) result in negative $\lambda_2 = 1-2p$. This determines the sign pattern of $(\lambda_2)^k$ in the spectral decomposition. Full analysis in Appendix~\ref{appendix:theory:empirical}.
\end{proof}

While a complete theoretical characterization for scenarios with multiple labels and varying homophily degrees remains an open challenge, our analysis provides rigorous justification for the empirical findings in Section~\ref{sec:empirical}. The convergence theory explains the universal label consistency decay observed across all graphs, while the eigenvalue analysis of transition matrices elegantly characterizes why homophilic and heterophilic graphs exhibit qualitatively different decay behaviors. This theoretical foundation deepens our understanding of how graph structure shapes label distributions and their evolution under random walks, providing principled support for our subsequent modeling approach.

==> experiment-number-temp.tex <==
\begin{table*}[!t]
    \centering
    \scriptsize
    \begin{threeparttable}
    \setlength{\tabcolsep}{0.15mm}{
    \begin{tabular}{@{}lccccccc|c@{}}
        \toprule
        \textbf{Method}                   &   \textbf{Cora}   &   \textbf{Citeseer}   &   \textbf{Pubmed} &   \textbf{WikiCS}     &   \textbf{Computers}  &   \textbf{Photo}      &   \textbf{Co.CS} &  \textbf{Rank}    \\ 
        \midrule
        GCN                 &   $81.5$          &   $70.3$              &   $79.0$          &   $77.19 \pm 0.12$    &   $86.51 \pm 0.54$    &   $92.42 \pm 0.22$    &   $93.03 \pm 0.31$ &  16.7  \\
        GAT                 &   $83.0 \pm 0.7$  &   $72.5 \pm 0.7$      &   $79.0 \pm 0.3$  &   $77.65 \pm 0.11$    &   $86.93 \pm 0.29$    &   $92.56 \pm 0.35$    &   $92.31 \pm 0.24$ &   14.4 \\
        GAE                        &   $71.5 \pm 0.4$  &   $65.8 \pm 0.4$      &   $72.1 \pm 0.5$  &   $70.15 \pm 0.01$    &   $85.27 \pm 0.19$    &   $91.62 \pm 0.13$    &   $90.01 \pm 0.71$ &  21.4 \\
        VGAE                          &   $76.3 \pm 0.2$  &   $66.8 \pm 0.2$      &   $75.8 \pm 0.4$  &   $75.63 \pm 0.19$    &   $86.37 \pm 0.21$    &   $92.20 \pm 0.11$    &   $92.11 \pm 0.09$ &  19.7  \\ 
        GraphMAE                       &   $84.2 \pm 0.4$  &   $73.4 \pm 0.4$      &   $81.1 \pm 0.4$  &   $77.12 \pm 0.30$                   &   $79.44 \pm 0.48$                   &   $90.71 \pm 0.40$                  &   $93.13 \pm 0.15$       &     11.9     \\
        DGI                           &   $82.3 \pm 0.6$  &   $71.8 \pm 0.7$      &   $76.8 \pm 0.6$  &   $75.35 \pm 0.14$    &   $83.95 \pm 0.47$    &   $91.61 \pm 0.22$    &   $92.15 \pm 0.63$ &  19.0 \\
        MVGRL              &   $83.5 \pm 0.4$  &   $73.3 \pm 0.5$      &   $80.1 \pm 0.7$  &   $77.52 \pm 0.08$    &   $87.52 \pm 0.11$    &   $91.74 \pm 0.07$    &   $92.11 \pm 0.12$   & 13.6 \\
        GRACE                        &   $81.9 \pm 0.4$  &   $71.2 \pm 0.5$      &   $80.6 \pm 0.4$  &   $78.19 \pm 0.01$    &   $86.25 \pm 0.25$    &   $92.15 \pm 0.24$    &   $92.93 \pm 0.01$   &  15.4 \\
        GCA                           &   $82.1 \pm 0.1$  &   $71.3 \pm  0.4$     &   $80.2 \pm 0.4$  &   $78.30 \pm 0.00$    &   $87.85 \pm 0.31$    &   $92.49 \pm 0.09$    &   $93.10 \pm 0.01$    & 13.7  \\
        BGRL                         &   $82.7 \pm 0.6$  &   $71.1 \pm 0.8$      &   $79.6 \pm 0.5$  &   $79.31 \pm 0.55$    &   $89.62 \pm 0.37$    &   $93.07 \pm 0.34$    &   $92.67 \pm 0.21$    & 11.7 \\
        G-BT                         &   $81.5 \pm 0.4$               &   $71.9 \pm 0.5$                 &   $80.4 \pm 0.6$               &   $76.65 \pm 0.62$    &   $88.14 \pm 0.33$    &   $92.63 \pm 0.44$    &   $92.95 \pm 0.17$     &  14.3 \\   
        CCA-SSG                        &   $84.2 \pm 0.4$  &   $73.1 \pm 0.3$      &   $81.6 \pm 0.4$  &   $78.65 \pm 0.14$                   &   $88.74 \pm 0.28$    &   $93.14 \pm 0.14$    &   $93.31 \pm 0.22$    &  6.4 \\
        gCooL                  &  $83.2\pm0.5$    &    $72.7\pm0.4$     &   $80.5\pm0.4$  &     $78.74 \pm 0.04$  &    $88.85 \pm 0.14$   &   $93.18 \pm 0.12$    &    $93.32 \pm 0.02$      &   8.3     \\
        HomoGCL                         &   $ \mathbf{84.5\pm0.5} $               &   $ 72.3\pm 0.7$                   &   $ 81.1\pm 0.3$               &   $ 78.84\pm0.47 $    &   $ 88.46\pm0.20 $    &   $ 92.92\pm0.18 $    &   $ 92.74\pm0.22 $  
  & 8.9 \\         
        COSTA                          &   $83.3 \pm 0.3$               &   $72.1 \pm 0.3$                   &   $81.1 \pm 0.2$               &   $79.12 \pm 0.02$    &   $88.32 \pm 0.03$    &   $92.56 \pm 0.45$    &   $92.94 \pm 0.10$   & 9.7 \\
        SUGRL                          &   $83.4 \pm 0.5$  &   $73.0 \pm 0.4$      &   $81.9 \pm 0.3$  &   $78.97 \pm 0.22$                  &   $88.91 \pm 0.22$      &   $92.85 \pm 0.24$      &   $92.83 \pm 0.23$           &    7.9   \\ 
        AFGRL                         &   $83.2 \pm 0.4$               &   $72.6 \pm 0.3$                   &   $80.8 \pm 0.6$               &   $77.62 \pm 0.49$    &   $89.88 \pm 0.33$    &   $93.22 \pm 0.28$    &   $93.27 \pm 0.17$  
  & 8.0 \\         
        SP-GCL                          &   $83.2 \pm 0.2$  &   $72.0 \pm 0.4$     &   $79.1 \pm 0.8$  &   $79.01 \pm 0.51$                &   $89.68 \pm 0.19$     &   $92.49 \pm 0.31$     &   $91.92 \pm 0.10$         &   12.6    \\ 
        GraphACL               &   $84.2\pm0.3$  &   $73.6\pm0.2$     &  $82.0\pm0.2$   &        $79.27 \pm 0.45$           &    $89.80\pm0.25$    &     $93.31\pm0.19$   &    $92.77 \pm 0.14$        &  \underline{5.3}    \\ 
        AUTOSSL                           &   $83.1 \pm 0.4$  &   $72.1 \pm 0.4$     &   $80.9 \pm 0.6$  &   $76.80 \pm 0.13$    &   $88.18 \pm 0.43$    &   $92.71 \pm 0.32$    &   $93.35 \pm 0.09$    & 11.0  \\   
        \midrule
       \rowcolor{gray!20} \mymodel{}\textsubscript{\textsc{Pair}}        &  \underline{$84.4 \pm 0.2$}  &   $\mathbf{73.7 \pm 0.4}$     &   \underline{$82.2 \pm 0.3$}  &   \underline{$80.14 \pm 0.51$}    &   $\mathbf{90.14 \pm  0.35}$    &   $\mathbf{93.42 \pm 0.44}$    &   $\mathbf{93.53 \pm 0.12}$  &  $\mathbf{1.6}$ \\
       \rowcolor{gray!20}  \mymodel{}\textsubscript{\textsc{List}}                &   $\mathbf{84.5 \pm 0.4}$  &   \underline{$73.6 \pm 0.5$}      &   $\mathbf{82.7 \pm 0.4}$  &   $\mathbf{80.16 \pm 0.58}$    &   \underline{$89.99 \pm  0.38$}    &   \underline{$93.40 \pm 0.48$}    &   \underline{$93.50 \pm 0.12$}    &  $\mathbf{1.6}$ \\
        \bottomrule
    \end{tabular}}
    \end{threeparttable}
        \caption{Classification accuracies on 7 GCL benchmark datasets (mean$\pm$std). `Rank' refers to the average ranking of a method across the 7 datasets. \textbf{Bold} indicates the best performance and \underline{underline} indicates the runner-up.}
    \label{tab:main_results}
    \vspace{-0.25cm}
\end{table*}


\begin{table}[!t]
\centering
\scriptsize
\vspace{-3.0mm}
\setlength{\tabcolsep}{0.3mm}{
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Method} & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Actor} \\ \midrule
    DGI            &       $60.27 \pm 0.70$             &       $42.22 \pm 0.63$            &      $28.30 \pm 0.76$          \\
    GRACE            &       $61.24 \pm 0.53$             &      $41.09 \pm 0.85$             &       $28.27 \pm 0.43$         \\
    GCA            &        $60.94 \pm 0.81$            &      $41.53 \pm 1.09$             &      $28.89 \pm 0.50$          \\
    BGRL            &        $64.86 \pm 0.63$            &      $46.24 \pm 0.70$             &      $28.80 \pm 0.54$          \\
    AFGRL            &        $59.03 \pm 0.78$            &      $42.36 \pm 0.40$             &      $27.43 \pm 1.31$          \\
    SP-GCL            &      $65.28 \pm 0.53$              &      $52.10 \pm 0.67$             &     $28.94 \pm 0.69$           \\ 
    GraphACL            &        \underline{$69.12\pm0.24$}           &        $54.05\pm0.13$            &       $30.03\pm0.13$         \\
    \midrule
    \rowcolor{gray!20} \mymodel{}\textsubscript{\textsc{Pair}}            &        $\mathbf{69.25 \pm 0.89}$            &      $\mathbf{57.67 \pm 0.96}$             &         $\mathbf{30.32 \pm 0.91}$       \\
    \rowcolor{gray!20} \mymodel{}\textsubscript{\textsc{List}}            &         $69.06 \pm 0.86$           &       \underline{$57.53 \pm 0.92$}            &        \underline{$30.23 \pm 0.88$}        \\
 \bottomrule
\end{tabular}}
\caption{Performance on 3 heterophily graph datasets.}
\label{tab:heter}
\vspace{-0.36cm}
\end{table}

\begin{table}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{0.3mm}{
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Method} & \textbf{Validation} & \textbf{Test}  \\ \midrule
    DGI            &       $71.26 \pm 0.11$             &       $70.34 \pm 0.16$                     \\
    GRACE-Sampling            &       $72.61 \pm 0.15$             &       $71.51 \pm 0.11$                  \\
    G-BT            &       $71.16 \pm 0.14$             &      $70.12 \pm 0.18$                    \\
    BGRL            &      $72.53 \pm 0.09$              &       $71.64 \pm 0.12$                     \\ 
    CCA-SSG            &      $72.34 \pm 0.21$              &       $71.24 \pm 0.20$                     \\ 
    GraphACL            &          $72.59\pm0.20$          &              $71.68\pm0.22$              \\     
    \midrule
    \rowcolor{gray!20} \mymodel{}\textsubscript{\textsc{Pair}}            &        \underline{$72.69 \pm 0.14$}                       &         \underline{$72.06 \pm 0.20$}       \\ 
    \rowcolor{gray!20} \mymodel{}\textsubscript{\textsc{List}}           &         $\mathbf{72.75 \pm 0.12}$                     &        $\mathbf{72.24 \pm 0.19}$        \\
     \midrule
     Supervised GCN            &        $73.00 \pm 0.17$            &        $71.74 \pm 0.29$                   \\ 
    \bottomrule
\end{tabular}}
\caption{Performance on a large scale graph dataset ogbn-arxiv. }
\label{tab:ogb}
\vspace{-0.35cm}
\end{table}
